Learning Concise and Descriptive Attributes for Visual Recognition

Recent advances in foundation models present new opportunities for interpretable visual recognition -- one can first query Large Language Models (LLMs) to obtain a set of attributes that describe each class, then apply vision-language models to classify images via these attributes. Pioneering work shows that querying thousands of attributes can achieve performance competitive with image features. However, our further investigation on 8 datasets reveals that LLM-generated attributes in a large quantity perform almost the same as random words. This surprising finding suggests that significant noise may be present in these attributes. We hypothesize that there exist subsets of attributes that can maintain the classification performance with much smaller sizes, and propose a novel learning-to-search method to discover those concise sets of attributes. As a result, on the CUB dataset, our method achieves performance close to that of massive LLM-generated attributes (e.g., 10k attributes for CUB), yet using only 32 attributes in total to distinguish 200 bird species. Furthermore, our new paradigm demonstrates several additional benefits: higher interpretability and interactivity for humans, and the ability to summarize knowledge for a recognition task.

==> experiment_old.tex <==
\section{Experiments}
\begin{figure*}[ht]
\centering
\subfigure[CUB]{\label{fig:cub}\includegraphics[width=0.240\linewidth]{figures/cub_4_to_512_old.pdf}}
\hfill
\subfigure[CIFAR10]{\label{fig:cifar10}\includegraphics[width=0.240\linewidth]{figures/cifar10_4_to_512_old.pdf}}
\subfigure[CIFAR-100]{\label{fig:CIFAR-100}\includegraphics[width=0.240\linewidth]{figures/CIFAR100_4_to_512_old.pdf}}
\hfill
\subfigure[Flower]{\label{fig:flower}\includegraphics[width=0.240\linewidth]{figures/flower_4_to_512_old.pdf}}
\hfill
\subfigure[Food]{\label{fig:food}\includegraphics[width=0.240\linewidth]{figures/food_4_to_512_old.pdf}}
\subfigure[Oxford\_pets]{\label{fig:oxford_pets}\includegraphics[width=0.240\linewidth]{figures/oxford_pets_4_to_512_old.pdf}}
\subfigure[Stanford\_cars]{\label{fig:stanford_cars}\includegraphics[width=0.240\linewidth]{figures/cars_4_to_512_old.pdf}}
\subfigure[Imagenet\_Animals]{\label{fig:imagenet_animals}\includegraphics[width=0.240\linewidth]{figures/imagenet-animal_4_to_512_old.pdf}}
\caption{Overall Performance on all datasets. X-axis: number of attributes, Y-axis: Accuracy (\%), ``(f)" means ``full", \ie, all attributes in the pool are used. Uniform refers to uniform sampling. }
\label{fig:overall_performances}
\end{figure*}

% To illustrate the effectiveness of our method, we conduct extensive experiments to discuss and analyze our method in various aspects. We will start with the experimental setup, then present our main results, followed by ablation studies for each component, and finally the case studies to explore the interpretability and interactivitiy of our model in detail. 

\subsection{Experimental Setup}
\paragraph{Datasets} We conduct our experiments on 8 different image classification datasets, including: CUB~\cite{cub}, CIFAR-10 and CIFAR-100~\cite{cifar10}, Food-101~\cite{food}, Flower~\cite{flower}, Oxford-pets~\cite{oxford_pets}, Stanford-cars~\cite{stanford_cars}, Imagenet~\cite{imagenet}. For Imagenet, it is not trivial to analyze all 1000 diverse classes. So we narrow the scope to 397 animal classes, with 509,230/19,850 samples for train/test. 
%samples out of 1,281,167 and 50,000 images, respectively. 
We denote this subset as Imagenet-Animals. For other datasets, most of them include images within a specific domain (CUB, Flower, Food, Oxford-pets, Stanford-cars), while CIFAR-10 and CIFAR-100 contain broader classes that lie across domains. 

\vspace{-8pt}
\paragraph{Implementation Details}
Our method involves two stages of training. The first stage consists of task-guided learning of a dictionary $\textbf{E}$ to approximate CLIP text embeddings and using this dictionary to find $K$ attributes for visual recognition. For the Mahalanobis distance, the parameter $\lambda$ is tuned with a grid search in \{1, 0.1, 0.01, 0.001, 0\}. The second stage is one-layer linear probing to classify semantic vectors. 
The batchsize is set to 4,096 for all datasets except 32,768 on Imagenet-Animals for faster converging. We set the number of epochs to 5,000 epochs with early stopping. 
% \wy{chatgpt: The batch size has been configured to 4096 for all datasets, except for Imagenet-Animals, where it has been set to 32768 to expedite the convergence process. Additionally, we have designated a total of 5000 epochs with an early stopping mechanism.}
The learning rate is set to 0.01 in all experiments with an Adam optimizer~\cite{kingma2014adam}. Unless specified, we use GPT-3 and CLIP ViT-B/32 for all performance comparison.

\vspace{-8pt}
\paragraph{Baselines}
We compare with state-of-the-art works that leverage attributes either from human annotations or from LLMs. For a fair comparison, we use linear probes to evaluate all methods: (1)~\textbf{CompDL}~\cite{compDL} builds semantic vectors using CLIP scores between human-designed attributes and images. (2)~\textbf{LaBO}~\cite{yang2022language} is a recent work that builds semantic vectors with a large set of attributes from LLMs. (3)~\textbf{Human}~\cite{cub,koh2020concept}. Attribute labels for each image are annotated by humans. We compare with two versions: binary labels for each attribute, and calibrated labels with confidence scores given by annotators.

To validate the effectiveness of learning-to-search, we explore other baselines: (1)~\textbf{K-means}. Perform K-means clustering on CLIP attribute embeddings, then find $K$ attributes with nearest distance to each clustering center. Intuitively this can be a strong baseline, as $K$ attributes close to each center can be distinctive.  (2)~\textbf{Uniform Sampling} from the large attribute pool.  (3)~\textbf{SVD}. After obtaining the attribute embeddings $\textbf{T}$, we run SVD decomposition of $\textbf{T}$ to get the top $K$ vectors and find attributes with the largest similarity with the $K$ important vectors. (4)~\textbf{Similarity}. We calculate the average score of each attribute across all images and then find the $K$ attributes with the largest average scores. (5) \textbf{Img Features}. Black-box linear probing on latent image features with two linear layers and an intermediate dimension $K$ as a reference.
% \subsection{Ablation study with Random Words}

% \begin{figure}
% \centering
% \subfigure[CUB]{\label{fig:cub}\includegraphics[width=0.480\linewidth]{figures/cub_scale.pdf}}
% \hfill
% \subfigure[Flower]{\label{fig:cifar10}\includegraphics[width=0.480\linewidth]{figures/flower_scale.pdf}}
% \caption{Performances with Random Words}
% \label{fig:overall_performances_with_random_words}
% \end{figure}
\subsection{Main Results}
\paragraph{Number of attributes and selection methods}.
We present our results in~\cref{fig:overall_performances}. 
First, our method is competitive with image features when $K$ is large. Reducing number of attributes $K$ to the number of classes $C$ (e.g., 512 to 128 for CUB) does not significantly hurt classification performance, even for baseline selection methods. This validates our hypothesis that there is plenty of redundant information in the semantic space when the number of attributes is large (as used in LaBO~\cite{yang2022language}). It is possible to find a subset of expressive attributes for visual recognition. 
Second, our method also consistently outperforms other methods such as K-means clustering and uniform sampling, demonstrating the effectiveness of our task-guided searching method. 
Third, a heuristic design such as K-means performs similar as uniform selection.
% there is still a gap between our method and  latent image features, which is a reasonable trade-off between interpretability and classification performance but indicates potential for improvement in the future.

\vspace{-8pt}
\paragraph{Comparison with previous work.}
\begin{table}[]
    \centering
    \resizebox{0.9\linewidth}{!}{%
    \begin{tabular}{c|ccc|ccc}
    \toprule
        Datasets & \multicolumn{3}{c|}{CUB} & \multicolumn{3}{c}{CIFAR-100} \\
        \midrule
        $K$ & 32 & 200 & 400 & 64 & 100 & 200\\
        \midrule
        LaBo~\cite{yang2022language} & -- & 60.93 & 62.61 & -- & 75.10 &  76.94 \\
        Ours & 60.27 & \textbf{63.88} & \textbf{64.72} & 73.31 &\textbf{75.12} & \textbf{77.29} \\
        \midrule
        Datasets & \multicolumn{3}{|c|}{CUB (1 shot)} & \multicolumn{3}{c}{CUB (5 shot)} \\
        \midrule
        % $K$ & 32 & 64 & 200 & 400 & 32 & 64 & 200 & 400 \\
        $K$ & 64 & 200 & 400 & 64 & 200 & 400 \\
        \midrule
        LaBo &  -- & 15.79 & 16.43 &  -- & 40.74 & 42.31 \\
        % Ours & 14.45 & 15.93 & \textbf{17.31} & \textbf{17.21} & 38.18 & 40.69 & \textbf{44.16} &  \textbf{43.48}  \\
        Ours & 15.93 & \textbf{17.31} & \textbf{17.21} & 40.69 & \textbf{44.16} &  \textbf{43.48}  \\
        \bottomrule 
    \end{tabular}}
    \caption{Comparison with state-of-the-art methods. LaBo is designed to use at least as many attributes as classes.
    % the attributes with amount no less than the number of classes. 
    We use ``--" to denote non-applicability.}
    \vspace{-10pt}
\label{tab:comparison_with_labo}
\end{table}
We first compare our method with LaBo~\cite{yang2022language}. It is designed to use $M_c$ concepts per class with default number of 50, which corresponds to 10,000 attributes for CUB.
%and is way more than ours. 
For fair-comparison, we set $M_c$ as 1 and 2 in the experiments.
 As shown in~\cref{tab:comparison_with_labo}, our method outperforms LaBo with the same number of attributes on both the full and few-shot setting. Furthermore, our method can achieve similar accuracy with only a smaller number of attributes (e.g., 32 attributes for CUB). These results suggest that our learned attributes are discriminative enough to classify the images, despite given fewer attributes.

% Besides, we also conduct some experiments on CUB with few shot settings following LABO~\cite{yang2022language}. The results are also shown in Table \ref{tab:comparison_with_labo}. 


% \begin{table}[h!]
%     \centering
%     \resizebox{\linewidth}{!}{%
%     \begin{tabular}{c|cccc|cccc}
%     \toprule
%         Datasets & \multicolumn{4}{|c|}{CUB (1shot)} & \multicolumn{4}{c}{CUB (5shot)} \\
%         \midrule
%         $K$ & 32 & 64 & 200 & 400 & 32 & 64 & 200 & 400 \\
%         \midrule
%         LaBo & -- & -- & 15.79 & 16.43 & -- & -- & 40.74 & 42.31 \\
%         Ours & 14.45 & 15.93 & \textbf{17.31} & \textbf{17.21} & 38.18 & 40.69 & \textbf{44.16} &  \textbf{43.48}  \\
%         % Run without mahalanobis
%         \bottomrule 
%     \end{tabular}}
%     \caption{Performance Comparison in Few-shot situations.}
% \label{tab:comparison_with_labo_few_shot}
% \end{table}



% An
\begin{table}[t]
    \centering
    \resizebox{1.0\linewidth}{!}
    {%
    \begin{tabular}{l|cccc}
    \toprule
        % & \multicolumn{3}{c}{K}\\
        % \midrule
        K (\# of attributes) & 8 & 16 & 32 & 312\\
        \midrule
        Human Binary~\cite{cub} & 4.02 & 7.31  & 10.11 & 47.38\\
        Human Calibration~\cite{koh2020concept}  & 3.75 & 7.15 & 9.78 & 43.37\\
        CompDL~\cite{compDL} & 12.64  &  26.41 &  28.69 & 52.60 \\
        Ours & \textbf{31.67}  & \textbf{48.55} & \textbf{60.27} & \textbf{65.17} \\
        % CLIP ViT-B/32 & 31.67  & 48.55 & 60.27 & 65.17 \\
        % CLIP ViT-L/14@336px  & 40.95 & 66.58  & 76.04 & 81.20\\
        \bottomrule 
    \end{tabular}}
    \caption{Comparison with human annotations on CUB.}
    \vspace{-10pt}
\label{tab:cub_human}
\end{table}
We then further compare with human annotations from CUB.  For $K<312$, we select attributes based on their accumulated confidence score for all samples. As shown in~\cref{tab:cub_human}, human annotated attributes are more noisy than CLIP similarities. With the same attributes, CLIP scores from CompDL build more expressive features. 
%On top of that, 
Furthermore,
our LLM-suggested attributes significantly outperform human designs, 
%it is able to use 
e.g.~by using
16 attributes we achieve similar performance as 312 attributes defined by humans.

\subsection{Ablation Study}
\label{sec:ablation}
\paragraph{GPT-3 vs Random or Similar words}
% \begin{figure}
% \begin{floatrow}
% \ffigbox{%
%   % \rule{3cm}{3cm}%
%   \includegraphics[width=\linewidth]{figures/cub_scale.pdf}
% }{%
%   \caption{Comparison with Random or Similar Words}%
%   \label{fig:compare_gpt3_random_similar}
% }
% \capbtabbox{%
% \resizebox{1.0\linewidth}{!}{%
%   \begin{tabular}{c|c} 
%   \toprule
%    & Examples \\
%   \midrule
%   \multirow{3}{*}{R} & \texttt{boy champagne} \\
%   % & {\footnotesize \texttt{condos journal information lexington designs}} \\
%   & \texttt{allied whose acrobat}\\
%   % & \\
%   & {\footnotesize \texttt{eight centered lobby heads} }\\
%   \midrule
%   \multirow{3}{*}{S} & \texttt{red,gray,snow wings} \\
%   & \texttt{orange wings} \\
%   & \texttt{lime,navy wings} \\
%   \midrule
%   \multirow{3}{*}{LM} & \texttt{sloping forehead}\\  
%   & \texttt{distinctive white throat} \\
%   & \texttt{bright red head and breast} \\
%   \bottomrule
%   \end{tabular}}
% }{%
%   \caption{Attribute instances from three different pools.}%
% }
% \end{floatrow}
% \end{figure}

\begin{figure}
    \centering
    \begin{minipage}{0.48\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/cub_scale.pdf}
    \caption{Performance comparison with random or similar words on CUB.}
    \label{fig:compare_gpt3_random_similar}
    \end{minipage}%
    \hfill
    \begin{minipage}{0.47\linewidth}
    \centering
    \captionsetup{type=table} %% tell latex to change to table
    \resizebox{1.0\linewidth}{!}{%
  \begin{tabular}{c|c} 
  \toprule
   & Examples \\
  \midrule
  \multirow{3}{*}{R} & \texttt{boy champagne} \\
  % & {\footnotesize \texttt{condos journal information lexington designs}} \\
  & \texttt{allied whose acrobat}\\
  % & \\
  & {\footnotesize \texttt{eight centered lobby heads} }\\
  \midrule
  \multirow{3}{*}{S} & \texttt{red,gray,snow wings} \\
  & \texttt{orange wings} \\
  & \texttt{lime,navy wings} \\
  \midrule
  \multirow{3}{*}{G} & \texttt{sloping forehead}\\  
  & \texttt{distinctive white throat} \\
  & \texttt{bright red head and breast} \\
  \bottomrule
  \end{tabular}}
    \caption{Examples from Random (R), Silimlar (S), GPT-3 (G) attributes}\label{tab:attribute_instances_from_different_pools}
    \end{minipage}
\end{figure}


We compare our method with random and similar words. As shown in~\cref{fig:compare_gpt3_random_similar}, when $K=512$, random words perform as well as GPT-3 attributes. 
Even reducing $K$ from 512 to 256 does not significantly hurt its performance. 
But when $K$ is small (e.g., 64), the performance of random words drops dramatically.
We conjecture that it is because text embeddings randomly drawn from CLIP are nearly orthogonal bases~\cite{wang2021average}. Given an image feature $\in \mathbb{R}^D$, projection with a set of $K$=$D$ orthogonal bases can perfectly preserve its information. 
We further explore how similar words (e.g., red wings, yellow wings) behave. Embeddings of similar words in a trained language model are not orthogonal bases hence the projection will lose information when $K$ is large. But as $K$ gets smaller, since those similar words have close semantic meanings, they start to outperform random words.
Overall, these finding motivate us to find a concise set of meaningful attributes while maintaining competitive performance.
% discriminativeness. 

% As the attributes generated by LLMs performs similar as the random words, this suggests that though these attributes are semantically meaningful, they are also diverse to the extent of random words. 

\vspace{-8pt}
\paragraph{Robustness to the attribute pool}
\begin{table}[]
    \centering
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{c|ccc|cccc}
        \toprule
        Datasets & \multicolumn{3}{|c|}{CUB} & \multicolumn{3}{c}{CIFAR-100} \\ 
        \midrule
        K & 8 & 16 & 32 & 8 & 16 & 32 \\
        \midrule
        GPT-3 & \textbf{31.67} & 48.55 & 60.27 & \textbf{34.77} & \textbf{52.24} & \textbf{66.30} \\
        GPT-3-Imagenet & 30.81 & \textbf{49.29} & \textbf{60.41} & 33.80 & 51.01 & 65.61 \\
%         ChatGPT & 21.66 & 40.28 & 47.46 & 
% 33.79 & 51.26 & \textbf{67.06} \\
        \bottomrule
    \end{tabular}}
    \caption{Ablation study \emph{w.r.t.} different concept pools.}
    \vspace{-8pt}
    \label{tab:gpt3_imagenet}
\end{table}

We aim to explore the effects of different concept pools generated by LLMs. We compare attributes from each dataset with attributes from the full set of ImageNet classes. As shown in~\cref{tab:gpt3_imagenet}, even with the large and noisy attributes from ImageNet,  our method can still efficiently find a small number of representative attributes for a task.

\vspace{-5pt}
\paragraph{Effectiveness of learning-to-search}
We discuss choices for selection out of the attribute pool in~\cref{tab:variation_of_attribute_selection} with the following observations: heuristic methods such as K-means and SVD are not  optimal choices for identifying the most distinctive attributes. In fact, they are sometimes less effective than uniform sampling. This is likely because we need to identify the most distinguishing attributes for visual recognition, rather than the most diverse ones based on text embeddings. Overall, our method significantly outperforms the other baselines, showing its efficacy. 
% Our method proves to be superior to the "Similarity" baseline, indicating that relying solely on the average relevance of attributes may not yield optimal results. Intuitively, the most distinct attributes are better suited for image classification, and they are not necessarily the most relevant. (3) 


\begin{table}[]
    \centering
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{c|ccc|cccc}
        \toprule
        Datasets & \multicolumn{3}{|c|}{CUB} & \multicolumn{3}{c}{CIFAR-100} \\ 
        \midrule
        K & 8 & 16 & 32 & 8 & 16 & 32 \\
        \midrule
        K-means & 16.83 & 21.02 & 32.76 & 25.39 & 45.26 & 64.41 \\
        Uniform & 7.02 & 25.98 & 40.58 & 28.07 & 47.14 & 64.34 \\
        SVD & 6.52 & 20.02 & 35.83 & 29.06 & 50.00 & 64.99\\
        Similarity & 4.73 & 9.72 & 18.00 &26.75 & 45.61 & 62.79 \\
        Ours & \textbf{31.67} & \textbf{48.55} & \textbf{60.27} & \textbf{34.77} & \textbf{52.24} & \textbf{66.30} \\
        \bottomrule
    \end{tabular}}
    \caption{Ablation study \emph{w.r.t.} different attribute selection strategies.}
    \label{tab:variation_of_attribute_selection}
\end{table}
\vspace{-8pt}
\paragraph{Effectiveness of regularization}
% Yu
We compare the Mahalanobis distance (\textit{MAH}) with two variations: (1) \textit{COS}: For each vector $\textbf{E}_j$ and $\textbf{T}_i$ (of the $i$-th attribute) in the concept pool, we computed averaged cosine distance as follows:
\begin{align*}
    \mathcal{L}_{cos} &= \frac{1}{K^2}\sum_{j=1}^K \sum_{i=1}^K \frac{\Trans{\textbf{T}}_i \textbf{E}_j}{||\textbf{T}_i|| || \textbf{E}_j||}
\end{align*}
(2) \textit{CE}: Learning with~\cref{eq:loss_cc} only.
Results are in~\cref{tab:variation_of_regularization}. Overall, Mahalanobis distance is an effective constraint to encourage the dictionary $E$ to be close to the distribution of CLIP embeddings.
\begin{table}[]
    \centering
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{c|cccc|cccc}
        \toprule
        Datasets & \multicolumn{4}{|c|}{CUB} & \multicolumn{4}{c}{CIFAR-100} \\ 
        \midrule
        K & 8 & 16 & 32 & 64 & 8 & 16 & 32 & 64 \\
        \midrule
        \textit{MAH} & 30.76 & 47.87 & \textbf{60.27} & \textbf{64.25} & \textbf{34.77} & \textbf{52.24} & 65.91 & \textbf{73.31} \\
        \textit{COS} & 28.96 & 47.35 & 58.27 & 63.25 & 31.98 & 51.15 & 65.02 &  72.80\\
        % $\mathcal{L}_2$ & 28.96 & 47.35 & 55.68 & 60.39 & 31.98 & 51.15 & 65.02 &  72.80 \\
        \textit{CE} & \textbf{31.67} & \textbf{48.55} & 55.88 & 60.73 & 32.45 & 50.83 & \textbf{66.29} & 73.25 \\
        \bottomrule
    \end{tabular}}
    \caption{Ablation study \emph{w.r.t.} different regularization.}
    \label{tab:variation_of_regularization}
\end{table}
\vspace{-5pt}



\subsection{Analysis of Interpretability and Interactivity}

\begin{figure*}
\subfigure[Least Auklet]
{\label{fig:least_auklet}\includegraphics[width=0.475\linewidth]{figures/least_auklet.pdf}}
\subfigure[Yellow Billed Cuckoo]{\label{fig:yellow_billed_cuckoo}\includegraphics[width=0.475\linewidth]{figures/yellow_billed_cuckoo.pdf}}
\caption{Examples on interpretability and interactivity. (1)~The upper half of each figure show important attributes for two classes of birds. We choose 6 out of 32 attributes with highest importance scores, which are computed by multiplication between clip scores and weights in the linear probe, defined in~\cref{eqn:importance_score}. 
% while the scores are the element-wise multiplication of the semantic vector (consists of clip similarity scores) and the class-related row in the weight of the FC layer in linear probing. 
(2)~The lower half of each figure demonstrates the intervention on the semantic vector (i.e., CLIP scores) to correct the prediction, we use $\delta$=0.03 for all interventions on clip scores as an empirical value. The array of 6 scores are of the same order as the attributes.}
\vspace{-8pt}
\label{fig:test_time_intervene}
\end{figure*}


\noindent We perform analysis and visualizations to show that: \\
(1) \textbf{Our learned attributes provide interpretability}. 
As shown in~\cref{fig:test_time_intervene}, the upper half presents the images in a class $c$ and high relevant attributes to recognize them. 
Specifically, we denote $\textbf{W} \in \mathbb{R}^{K_C*K}$ as the weight of the FC layer in linear probing, where $K_C$, $K$ are the number of classes and attributes. 
Then for each image $i$ and its semantic vector $\textbf{A} \in \mathbb{R}^K$, 
we multiply the corresponding score vector of image $i$ with the corresponding row of the FC layer $\textbf{W}_c$ to compute Importance Score $\textbf{IS} \in \mathbb{R}^{K}$:
\begin{equation}
    \textbf{IS} = \textbf{W}_c \otimes \textbf{A}
\label{eqn:importance_score}
\end{equation}
where $\otimes$ means element-wise multiplication. Then we present attributes with the top absolute values of $\textbf{IS}$ averaged over all samples in a class, with blue/orange bars indicating the positive/negative importance. 
% Since all CLIP scores~\cite{hessel2021clipscore} are positive, our linear probe also gains interpretability, as classes with larger logits indicate higher probabilities for prediction.
% Note that higher absolute values mean higher importance, while positive ones means this attribute is important to the class, while negative ones indicate that this image should not be classified as this class if it's highly aligned with the current attribute.
Higher absolute values denote greater significance. Since all CLIP scores are positive~\cite{hessel2021clipscore}, the positivity or negativity of high IS signifies their relevance to the class.

\noindent (2) \textbf{Our concise set of attributes enables simple interactivity}. As shown in the lower half of~\cref{fig:test_time_intervene}, we can correct the model's wrong predictions during inference by changing only a single similarity score between an image and the attribute that the CLIP model made a mistake on. This is a significant simplification compared with previous work~\cite{koh2020concept} where they need to manipulate scores from a group of concepts for the CUB dataset. We present more user studies in~\cref{app:case_study}.

% This shows that human could interact with the model by intervening on the similarity scores to help the model make right predictions. 
% We present more case studies in Appendix \ref{app:case_study}



% Manipulating the concept scores during test time: Say an image with bird-A is classified as bird-B by our model, by changing some similarity scores in the vector, we can correct the model's prediction back to bird-A. 

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{figures/least_auklet.pdf}
%     \caption{Important attributes for Least Auklet out of 32 attributes and the intervention on the clip score in the dataset.}
%     \label{fig:least_auklet}
% \end{figure}
% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{figures/yellow_billed_cuckoo.pdf}
%     \caption{Important attributes for Yellow Billed Cuckoo out of 32 attributes and the intervention on the clip score in the dataset.}
%     \label{fig:yellow_billed_cuckoo}
% \end{figure}

\subsection{Visualization of Our Discovered Attributes}
\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{figures/features_8_out_of_16.pdf}
    \caption{A concise set of 8 descriptive attributes learned for each dataset with sampled images.}
    \label{fig:pruned_features}
\end{figure*}

We show our learned descriptive attributes with $K=8$ in~\cref{fig:pruned_features}. Intuitively, we can observe these attributes are distinctive for each domain. Take birds recognition (CUB) as an example, the eight attributes covered most of the body parts of a bird (head, breast, legs, etc.). As we are condensing knowledge from hundreds of bird classes, each attribute broadly covers many categories. A bright red head and breast can be a noticeable visual attribute for many bird species, such as the Northern Cardinal and the Vermilion Flycatcher. Overall, explaining a domain with a few descriptive attributes is challenging, even for an expert with sufficient domain knowledge. But our model is able to automatically provide a level of knowledge to help humans understand how visual recognition works. 

We then present case studies on CIFAR-10 with 4 attributes and CLIP scores of 10 random images from each class in~\cref{fig:cifar10_case_study}.
In general, each image is activated in an distinguishable way in the heat map. Some attributes can distinguish a few classes, for example, cat and dog have higher activation on ``fur coat'' compared to automobile or truck. Thus ``fur coat'' may be an important feature to differentiate animals and vehicles.
% These results suggest that our method can effectively identify the descriptive attributes that distinguish different types of objects.


\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/cifar10_case_study_with_bar.pdf}
    \vspace{-8pt}
    \caption{Case study on CIFAR-10. The numbers are CLIP similarity scores between each image and attributes.}
    \label{fig:cifar10_case_study} 
\end{figure}

% \paragraph{Similarity scores under adversarial attack / adding noises}
